On the performance of high-order finite elements with respect to maximum principles and the non-negative constraint for diffusion-type equations

The main aim of this paper is to document the performance of $p$-refinement with respect to maximum principles and the non-negative constraint. The model problem is (steady-state) anisotropic diffusion with decay (which is a second-order elliptic partial differential equation). We considered the standard single-field formulation (which is based on the Galerkin formalism) and two least-squares-based mixed formulations. We have employed non-uniform Lagrange polynomials for altering the polynomial order in each element, and we have used $p = 1, ..., 10$. It will be shown that the violation of the non-negative constraint will not vanish with $p$-refinement for anisotropic diffusion. We shall illustrate the performance of $p$-refinement using several representative problems. The intended outcome of the paper is twofold. Firstly, this study will caution the users of high-order approximations about its performance with respect to maximum principles and the non-negative constraint. Secondly, this study will help researchers to develop new methodologies for enforcing maximum principles and the non-negative constraint under high-order approximations.

==> Sections/LS_DMP_Figures_1D.tex <==
%************************************;
%                                    ;
%  NAME                              ;
%    S4_LS_DMP_High_order.tex        ;
%                                    ;
%************************************;

%----------------------------------;
%  Figure: High-order 1D elements  ;
%----------------------------------;
\begin{figure}
  \includegraphics[scale=0.6]{Figures/interp-p-6.eps}
  \caption{High polynomial order one-dimensional $C^0$ 
    Lagrange interpolation functions (cases shown are 
    for $p = 6$) with (a) equal spacing of the element 
    nodes, and (b) unequal nodal spacing associated with 
    Gauss-Lobatto-Legendre points. 
    \label{Fig:LS_DMP_high_order_1D}}
\end{figure}

%----------------------------------;
%  Figure: High-order 2D elements  ;
%----------------------------------;
\begin{figure}
  \includegraphics[scale=0.6]{Figures/spectral-elements.eps}
  \caption{Examples of various high-order two-dimensional 
    master elements $\hat {\Omega}^e$ used in the present 
    formulation: (a) four-node element ($p = 1$), (b) nine-node 
    element ($p = 2$), (c) twenty-five-node element ($p = 4$), 
    and (d) eighty-one-node element ($p = 8$). 
    \label{Fig:LS_DMP_high_order_2D}}
\end{figure}

%-----------------------------------------------------------;
%  Figure: 1D problem with zero forcing function: Galerkin  ;
%-----------------------------------------------------------;
\begin{figure}
  \includegraphics[scale=0.65]{MATLAB_codes/problem-01/fig-01-weak-h-p.eps}
  \caption{One-dimensional problem with zero forcing function: 
  The figure illustrates the performance of the classical 
  single-field formulation (which is also referred to as 
  the Galerkin formulation) with respect to the non-negative 
  constraint. In the right figure, we show the classical 
  single-field formulation with respect to $p$-refinement. 
  For comparison, the left figure shows the performance for 
  an equivalent $h$-refinement. For this test problem, the 
  violation of the non-negative constraint decreases with 
  both $h$- and $p$-refinements under the classical 
  single-field formulation. 
  \label{Fig:LS_DMP_1D_Galerkin_conc}}
\end{figure}

%------------------------------------------------------;
%  Figure: 1D problem with zero forcing function: LS1  ;
%------------------------------------------------------;
\begin{figure}
  \includegraphics[scale=0.65]{MATLAB_codes/problem-01/fig-02-lsfem-1-h-p.eps}
  \caption{One-dimensional problem with zero forcing function: 
    The figure illustrates the performance of the first-form of 
    the least-squares formulation (LS1 formulation) with respect 
    to the non-negative constraint. In the right figure, we show 
    the performance of the formulation with respect to $p$-refinement. 
    For comparison, the left figure shows the performance for an 
    equivalent $h$-refinement. For this problem, the violation 
    of the non-negative constraint decreases with both $h$- and 
    $p$-refinements under the LS1 formulation. 
    \label{Fig:LS_DMP_1D_first_LS_conc}}
\end{figure}

%------------------------------------------------------;
%  Figure: 1D problem with zero forcing function: LS2  ;
%------------------------------------------------------;
\begin{figure}
  \includegraphics[scale=0.65]{MATLAB_codes/problem-01/fig-03-lsfem-2-h-p.eps}
  \caption{One-dimensional problem with zero forcing function: 
    The figure illustrates the performance of the second-form of 
    the least-squares formulation (LS2 formulation). In the right 
    figure, we show the performance of the formulation due to 
    $p$-refinement. For comparison, the left figure shows the 
    performance for equivalent $h$-refinement. For this problem, 
    the violation of the non-negative constraint decreases with 
    both $h$- and $p$-refinements under the LS1 formulation.
    \label{Fig:LS_DMP_1D_second_LS_conc}}
\end{figure}

%---------------------------------------------------------------;
%  Figure: 1D problem with zero forcing function: LS2 and flux  ;
%---------------------------------------------------------------;
\begin{figure}
  \includegraphics[scale=0.65]{MATLAB_codes/problem-01/fig-04-lsfem-2-h-p.eps}
  \caption{One-dimensional problem with zero forcing function: 
  The figure shows the flux obtained using the second-form of 
  the least-squares formulation (LS2 formulation). In the right 
  figure, we show the performance of the formulation due to 
  $p$-refinement. For comparison, the left figure shows the 
  performance for equivalent $h$-refinement. 
  \label{Fig:LS_DMP_1D_no_forcing_flux}}
\end{figure}

%-------------------------------------------------------------------;
%  Figure: 1D problem with non-zero forcing function: LS2 and flux  ;
%-------------------------------------------------------------------;
\begin{figure}
  \subfigure{
    \includegraphics[scale=0.42]{MATLAB_codes/problem-02/prob-2-weak-p.eps}}
  \subfigure{
    \includegraphics[scale=0.42]{MATLAB_codes/problem-02/prob-2-lsfem-p.eps}}  
  \caption{One-dimensional problem with non-zero forcing function: 
    This figure shows the obtained concentration profiles for various 
    orders of polynomial approximations under the classical single-field 
    formulation (top figure) and the least-squares formulation (bottom 
    figure). 
    %
    Although $f(\mathbf{x}) \geq 0 \; \forall \mathbf{x} \in \Omega$, 
    both the classical single-field formulation (for $p = 3$) and the 
    least-squares formulation (for $p = 3$ and $p = 5$) violate the 
    non-negative constraint. 
    \label{Fig:LS_DMP_1D_homogeneous_Dirichlet}}
\end{figure}

==> Sections/LS_DMP_Figures_2D.tex <==
%************************************;
%                                    ;
%  NAME                              ;
%    S4_LS_DMP_High_order.tex        ;
%                                    ;
%************************************;

%==========================;
%  Figures for Problem #3  ;
%==========================;

%------------------------------;
%  Figure: Computational Mesh  ;
%------------------------------;
\begin{figure}
\subfigure{
    \includegraphics[scale=0.55]{MATLAB_codes/problem-03/mesh/prob-03-mesh.eps}}
\subfigure{
    \includegraphics[scale=0.55]{MATLAB_codes/problem-03/mesh/prob-03-mesh_visualization.eps}}
    %    
  \caption{Two-dimensional isotropic diffusion: The top figure shows the mesh 
  used in the numerical simulation, and the bottom figure shows the corresponding 
  mesh used for visualization under high-order approximations. For more details 
  on visualizing results using high-order approximations see subsection 
    \ref{Subsec:LS_DMP_visualization}.
  \label{Fig:LS_DMP_prob_3_mesh}}
\end{figure}

%----------------------------------------------------;
%  Figure: concentration under Galerkin formulation  ;
%----------------------------------------------------;
\begin{figure}
  \centering
  \includegraphics[scale=0.37]{MATLAB_codes/problem-03/weak/prob-3-weak-p1_p2_p5_p10.eps}
  \caption{Two-dimensional isotropic diffusion: This figure shows the 
    contours of the concentration obtained using the \emph{single-field 
      formulation} for various polynomial approximations. The top figures 
    are for $p = 1$ and $p = 2$, and the bottom figures are for $p = 5$ 
    and $p = 10$. The regions in which the non-negative constraint is 
    violated is shown in white color. 
    \label{Fig:LS_DMP_prob_3_weak_conc}}
\end{figure}

%-------------------------------------------------;
%  Figure: concentration under LSFEM formulation  ;
%-------------------------------------------------;
\begin{figure}
  \centering
  \includegraphics[scale=0.37]{MATLAB_codes/problem-03/lsfem/prob-3-lsfem-1-p1_p2_p5_p10.eps}
  \caption{Two-dimensional isotropic diffusion: This figure shows the 
    contours of the concentration obtained using the \emph{least-squares 
    formulation} for various polynomial approximations. The top figures 
    are for $p = 1$ and $p = 2$, and the bottom figures are for $p = 5$ 
    and $p =10$. (Since the diffusivity is isotropic and decay coefficient 
    is zero, both LS1 and LS2 formulations are identical.) The regions 
    in which the non-negative constraint is violated is shown in white 
    color. \label{Fig:LS_DMP_prob_3_lsfem_conc}}
\end{figure}

%%==========================;
%%  Figures for Problem #4  ;
%%==========================;

%%-----------------------------------------;
%%  Figure: Structured computational mesh  ;
%%-----------------------------------------;
%\begin{figure}
%  \centering
%  \subfigure{
%    \includegraphics[scale=0.4]{MATLAB_codes/problem-04/mesh/prob-4-struct-mesh.eps}}
%  \subfigure{
%    \includegraphics[scale=0.4]{MATLAB_codes/problem-04/mesh/prob-4-struct-mesh_visualization.eps}}
%  % 
%  \caption{Diffusivity tensor from the subsurface flow literature: The top 
%  figure shows the \emph{structured} mesh used in the numerical simulation, 
%  and the bottom figure shows the corresponding mesh used for visualization 
%  under high-order approximations. For more details on visualizing results 
%  using high-order approximations see subsection \ref{Subsec:LS_DMP_visualization}. 
%  \label{Fig:LS_DMP_prob_4_struct_mesh}}
%\end{figure}

%%-------------------------------------------;
%%  Figure: Unstructured computational mesh  ;
%%-------------------------------------------;
%\begin{figure}
%  \centering
%  \subfigure{
%    \includegraphics[scale=0.4]{MATLAB_codes/problem-04/mesh/prob-4-unstruct-mesh.eps}}
%  \subfigure{
%    \includegraphics[scale=0.4]{MATLAB_codes/problem-04/mesh/prob-4-unstruct-mesh_visualization.eps}}
%  % 
%  \caption{Diffusivity tensor from the subsurface flow literature: The top figure 
%  shows the \emph{unstructured} mesh used in the numerical simulation, and 
%  the bottom figure shows the corresponding mesh used for visualization under 
%  high-order approximations. For more details on visualizing results using 
%  high-order approximations see subsection \ref{Subsec:LS_DMP_visualization}. 
%  \label{Fig:LS_DMP_prob_4_unstruct_mesh}}
%\end{figure}

%==========================;
%  Figures for Problem #5  ;
%==========================;

%-----------------------------------------;
%  Figure: Computational structured mesh  ;
%-----------------------------------------;
\begin{figure}
  \centering
  \subfigure{
    \includegraphics[scale=0.4]{MATLAB_codes/problem-05/mesh/prob-5-struct_mesh.eps}}
  \subfigure{
    \includegraphics[scale=0.4]{MATLAB_codes/problem-05/mesh/prob-5-struct_mesh_visualization.eps}}
  % 
  \caption{Non-uniform anisotropic media: The top figure shows the 
    \emph{structured} mesh used in the numerical simulation, and the 
    bottom figure shows the corresponding mesh used for visualization 
    under high-order approximations. For more details on visualizing 
    results using high-order approximations see subsection 
    \ref{Subsec:LS_DMP_visualization}. 
    \label{Fig:LS_DMP_prob_5_struct_mesh}}
\end{figure}

%-------------------------------------------;
%  Figure: Computational unstructured mesh  ;
%-------------------------------------------;
\begin{figure}
  \centering
  \subfigure{
    \includegraphics[scale=0.4]{MATLAB_codes/problem-05/mesh/prob-5-unstruct_mesh.eps}}
  \subfigure{
    \includegraphics[scale=0.4]{MATLAB_codes/problem-05/mesh/prob-5-unstruct_mesh_visualization.eps}}
  % 
  \caption{Non-uniform anisotropic media: The top figure shows the 
    \emph{unstructured} mesh used in the numerical simulation, and 
    the bottom figure shows the corresponding mesh used for visualization 
    under high-order approximations. For more details on visualizing 
    results using high-order approximations see subsection 
    \ref{Subsec:LS_DMP_visualization}.
    \label{Fig:LS_DMP_prob_5_unstruct_mesh}}
\end{figure}

\clearpage
\newpage

%---------------------------------------------;
%  Figure: Weak formulation: Structured mesh  ;
%---------------------------------------------;
\begin{figure}
\centering
\includegraphics[scale=0.32]{MATLAB_codes/problem-05/weak/prob-5-weak-struct}
\caption{Non-uniform anisotropic media: 
This figure shows the concentration contours obtained using the 
\emph{single-field formulation} and structured mesh (which is 
show in Figure \ref{Fig:LS_DMP_prob_5_struct_mesh}). The 
left figures are using $h$-refinement, and the right figures are 
using $p$-refinement. The top figures are for $h/p = 2$, the 
middle figures are for $h/p = 5$, and the bottom two figures 
are for $h/p = 10$. \label{Fig:LS_DMP_prob_5_struct_weak}}
\end{figure}

%--------------------------------------------;
%  Figure: LS1 formulation: Structured mesh  ;
%--------------------------------------------;
\begin{figure}
  \centering
  \includegraphics[scale=0.32]{MATLAB_codes/problem-05/lsfem_1/prob-5-lsfem-1-struct.eps}
  \caption{Non-uniform anisotropic media: This figure shows the concentration 
  contours obtained using the \emph{LS1 formulation} and \emph{structured 
  mesh} (which is shown in Figure \ref{Fig:LS_DMP_prob_5_struct_mesh}). 
  The left figures are using $h$-refinement, and the right figures are using 
  $p$-refinement. The top figures are for $h/p = 2$, the middle figures are 
  for $h/p = 5$, and the bottom two figures are for $h/p = 10$. 
  \label{Fig:LS_DMP_prob_5_struct_lsfem_1}}
  \end{figure}

%--------------------------------------------;
%  Figure: LS2 formulation: Structured mesh  ;
%--------------------------------------------;
\begin{figure}
\centering
\includegraphics[scale=0.32]{MATLAB_codes/problem-05/lsfem_2/prob-5-lsfem-2-struct.eps}
\caption{Non-uniform anisotropic media: This figure shows the concentration 
contours obtained using the \emph{LS2 formulation} and \emph{structured 
mesh} (which is shown in Figure \ref{Fig:LS_DMP_prob_5_struct_mesh}). 
The left figures are using $h$-refinement, and the right figures are using 
  $p$-refinement. The top figures are for $h/p = 2$, the middle figures are 
  for $h/p = 5$, and the bottom two figures are for $h/p = 10$. 
  \label{Fig:LS_DMP_prob_5_struct_lsfem_2}}
\end{figure}

%-------------------------------------------------------------------;
%  Figure: Weak formulation: Unstructured mesh: Concentration plot  ;
%-------------------------------------------------------------------;
\begin{figure}
  \centering
  \includegraphics[scale=0.32]{MATLAB_codes/problem-05/weak/prob-5-weak-unstruct.eps}
  \caption{Non-uniform anisotropic media: This figure shows the 
    concentration contours obtained using the \emph{single-field 
      formulation} and \emph{unstructured mesh} (which is shown 
      in Figure \ref{Fig:LS_DMP_prob_5_unstruct_mesh}). The left 
      figures are using $h$-refinement, and the right figures are using 
      $p$-refinement. The top figures are for $h/p = 2$, the middle 
      figures are for $h/p = 5$, and the bottom two figures are for 
      $h/p = 10$. \label{Fig:LS_DMP_prob_5_unstruct_weak}}
\end{figure}

%----------------------------------------------;
%  Figure: LS1 formulation: Unstructured mesh  ;
%----------------------------------------------;
\begin{figure}
\centering
\includegraphics[scale=0.32]{MATLAB_codes/problem-05/lsfem_1/prob-5-lsfem-1-unstruct.eps}
\caption{Non-uniform anisotropic media: This figure shows the concentration 
contours obtained using the \emph{LS1 formulation} and \emph{unstructured 
mesh} (which is shown in Figure \ref{Fig:LS_DMP_prob_5_unstruct_mesh}). 
The left figures are using $h$-refinement, and the right figures are using 
  $p$-refinement. The top figures are for $h/p = 2$, the middle figures are 
  for $h/p = 5$, and the bottom two figures are for $h/p = 10$. 
\label{Fig:LS_DMP_prob_5_unstruct_LS1}}
\end{figure}

%----------------------------------------------------------;
%  Figure: Problem #5: LS2 formulation: Unstructured mesh  ;
%----------------------------------------------------------;
\begin{figure}
\centering
\includegraphics[scale=0.32]{MATLAB_codes/problem-05/lsfem_2/prob-5-lsfem-2-unstruct.eps}
\caption{Non-uniform anisotropic media: This figure shows the concentration 
contours obtained using the \emph{LS2 formulation} and \emph{unstructured 
mesh} (which is shown in Figure \ref{Fig:LS_DMP_prob_5_unstruct_mesh}). 
The left figures are using $h$-refinement, and the right figures are using 
  $p$-refinement. The top figures are for $h/p = 2$, the middle figures are 
  for $h/p = 5$, and the bottom two figures are for $h/p = 10$. 
\label{Fig:LS_DMP_prob_5_unstruct_LS2}}
\end{figure}

%----------------------------------------------------------------;
%  Figure: Problem #5: Violation of the non-negative constraint  ;
%----------------------------------------------------------------;
\begin{figure}
  \centering
  \subfigure{
    \includegraphics[scale=0.5]{MATLAB_codes/problem-05/min_conc/Problem_5_min_conc_struct_mesh.eps}}
  \subfigure{
    \includegraphics[scale=0.5]{MATLAB_codes/problem-05/min_conc/Problem_5_min_conc_unstruct_mesh.eps}}
  \caption{Non-uniform anisotropic media: This figure shows 
    the minimum concentration for various order of polynomial 
    approximation for single-field, LS1 and LS2 formulations 
    using structured (top figure) and unstructured (bottom 
    figure) meshes. According to the maximum principle, the 
    concentration should be non-negative and should occur on 
    the boundary. However, for all the three formulations the 
    obtained minimum concentration is negative. The violation 
    of the non-negative constraint did not vanish under either 
    $p$- or $h$-refinement. For better comparison, we have taken 
    the $y$-axis to be the logarithm of the negative of the minimum 
    concentration. \label{Fig:LS_DMP_prob_5_min_conc}}
\end{figure}

%==========================;
%  Figures for Problem #6  ;
%==========================;

%------------------------------;
%  Figure: Computational mesh  ;
%------------------------------;
\begin{figure}
  \centering
  \subfigure{
    \includegraphics[scale=0.4]{MATLAB_codes/problem-06/mesh/prob-6-unstruct-mesh.eps}}
  \subfigure{
    \includegraphics[scale=0.4]{MATLAB_codes/problem-06/mesh/prob-6-unstruct-mesh_visualization.eps}}
  % 
  \caption{Anisotropic diffusion in a square domain with a hole: The top figure 
  shows the mesh used in the numerical simulation, and the bottom figure 
  shows the corresponding mesh used for visualization under high-order 
  approximations. For more details on visualizing results using high-order 
  approximations see subsection \ref{Subsec:LS_DMP_visualization}. 
  \label{Fig:LS_DMP_prob_6_mesh}}
\end{figure}

%-----------------------------------------------;
%  Figure: k_2=10000, single-field formulation  ;
%-----------------------------------------------;
\begin{figure}
\centering
\includegraphics[scale=0.32]{MATLAB_codes/problem-06/weak/prob-6-weak-unstruct-k2_10000.eps}
\caption{Anisotropic diffusion in a square domain with a hole: 
  This figure shows the concentration contours obtained using 
  the \emph{single-field formulation} for $k_1 = 1$ and $k_2 = 
  10000$. The left figures are for $h$-refinement, and the right 
  figures are $p$-refinement. The top figures are for $h/p = 2$, 
  the middle figures are for $h/p = 5$, and the bottom two figures 
  are for $h/p = 10$. \label{Fig:LS_DMP_prob_6_k2_10000_Galerkin}}
\end{figure}

%--------------------------------------;
%  Figure: k_2=10000, LS1 formulation  ;
%--------------------------------------;
\begin{figure}
\centering
\includegraphics[scale=0.32]{MATLAB_codes/problem-06/lsfem_1/prob-6-lsfem-1-unstruct-k2_10000.eps}
\caption{Anisotropic diffusion in a square domain with a hole: 
  This figure shows the concentration contours obtained using 
  the \emph{LS1 formulation} for $k_1 = 1$ and $k_2 = 10000$. 
  The left figures are using $h$-refinement, and the right figures 
  using $p$-refinement. The top figures are for $h/p = 2$, the 
  middle figures are for $h/p = 5$, and the bottom two figures 
  are for $h/p = 10$. \label{Fig:LS_DMP_prob_6_k2_10000_LS1}}
\end{figure}

%--------------------------------------;
%  Figure: k_2=10000, LS2 formulation  ;
%--------------------------------------;
\begin{figure}
\centering
\includegraphics[scale=0.32]{MATLAB_codes/problem-06/lsfem_2/prob-6-lsfem-2-unstruct-k2_10000.eps}
\caption{Anisotropic diffusion in a square domain with a hole: 
  This figure shows the concentration contours obtained using 
  the \emph{LS2 formulation} for $k_1 = 1$ and $k_2 = 10000$. 
  The left figures are for $h$-refinement, and the right figures 
  are $p$-refinement. The top figures are for $h/p = 2$, the 
  middle figures are for $h/p = 5$, and the bottom two figures 
  are for $h/p = 10$. \label{Fig:LS_DMP_prob_6_k2_10000_LS2}}
\end{figure}

%----------------------------------------------------;
%  Figure: Violation of the non-negative constraint  ;
%----------------------------------------------------;
\begin{figure}
  \centering
  \subfigure{
    \includegraphics[scale=0.5]{MATLAB_codes/problem-06/min_conc/Problem_6_min_conc_k1_1_k2_1.eps}}
  % 
  \subfigure{
    \includegraphics[scale=0.5]{MATLAB_codes/problem-06/min_conc/Problem_6_min_conc_k1_1_k2_10000.eps}}
  % 
  \caption{Anisotropic diffusion in a square domain with a hole: 
    This figure shows the minimum concentration under single-field, 
    LS1 and LS2 formulations for two different cases: $k_1 = 1$ and 
    $k_2 = 100$ (top figure), and $k_1 = 1$ and $k_2 = 10000$ (bottom 
    figure). We have shown the minimum concentration under various 
    levels of $p$- and $h$-refinements. For all the three formulations 
    and under various levels of $p$- and $h$-refinements, the minimum 
    concentration is negative. 
    %
    For better comparison, we have taken the $y$-axis to be the 
    logarithm of the negative of the minimum concentration. (Note 
    that the minimum concentrations obtain using the single-field 
    and LS2 formulations are approximately the same under both 
    $p$- and $h$-refinements.) 
    \label{Fig:LS_DMP_prob_6_min_conc}}
\end{figure}


==> Sections/S1_LS_DMP_Introduction.tex <==
%*********************************************;
%                                             ;
%  NAME                                       ;
%    S1_LS_DMP_Introduction.tex               ;
%                                             ;
%*********************************************;
\section{INTRODUCTION}
\label{Sec:LS_DMP_Introduction}
Contaminant transport, chemical and biological remediation, and 
carbon-dioxide sequestration are some of the main engineering 
challenges of the 21st century. A large-scale implementation of 
any of these problems will have irreversible consequences on the 
environment, and can affect large geographical region and for 
long periods of time. In addressing these pressing issues, 
robust predictive numerical simulations have played and will 
continue to play an important role. 

In these kind of problems, predicting the fate of chemical species is an 
important component, and diffusion is a dominant phenomenon. It should 
be noted that concentration (and certain other quantities such as absolute 
temperature, density, absolute pressure, saturation in multiphase systems) 
attains only non-negative values. A negative value for the concentration 
is unphysical. In a coupled reactive-transport numerical simulator, a negative 
value for the concentration of a species will result in an algorithmic failure. 
A robust numerical simulation should therefore preserve the physical and 
mathematical requirement of non-negativeness of species concentration.

%================================================================;
%  Subsection: Maximum principles and high-order approximations  ;
%================================================================;
\subsection{Maximum principles and high-order approximations}
Mathematically speaking, steady-state diffusion-type equations are 
elliptic partial differential equations, and are known to satisfy 
the so-called \emph{maximum principles} \cite{Gilbarg_Trudinger}. 
The non-negative constraint can be obtained from maximum principles 
under certain assumptions on the input data. The discrete version 
of maximum principles are commonly referred to as {discrete maximum 
principles} (DMP). A study on discrete maximum principles investigates 
whether a given numerical formulation (that is, in a discrete setting) 
inherits the underlying maximum principles (which are satisfied in the 
continuous setting). A robust predictive numerical simulation should 
preserve various fundamental properties like the non-negativeness 
and maximum principles. Hence, one is particularly interested in 
the necessary and/or sufficient conditions under which a given 
numerical formulation satisfies discrete maximum principles and 
the non-negative constraint. 

Many numerical formulations (under finite element, finite volume, 
and finite difference methodologies) have been developed. However, 
it should \emph{not} be expected that any of these formulations 
will satisfy maximum principles and the non-negative constraint 
as there are no in-built mechanisms in these formulations to meet 
such constraints. Recently, researchers have proposed numerical 
methodologies for enforcing maximum principles and the non-negative 
constraint. 
%
For example, References 
\cite{Lipnikov_Shashkov_Svyatskiy_Vassilevski_JCP_2007_v227_p492,
Lipnikov_Svyatskiy_Vassilevski_JCP_2009_v228_p703} have addressed 
the non-negative constraint under the finite volume method. Liska 
and Shashkov \cite{Liska_Shashkov_CiCP_2008_v3_p852} have proposed 
a methodology to meet these constraints using the conservative 
finite difference technique. In References 
\cite{Nakshatrala_Valocchi_JCP_2009_v228_p6726,
Nagarajan_Nakshatrala_IJNMF_2010}, optimization-based techniques 
have been employed to meet these constraints under both mixed and 
single-field finite element formulations but have restricted their 
studies to low-order finite elements. 

One of the early studies on discrete maximum principles is due to Varga 
\cite{Varga_SIAMJNA_1966_v3_p355}, which was in the context of finite 
difference. An important work on discrete maximum principles with 
respect to the finite element method is by Ciarlet and Raviart 
\cite{Ciarlet_Raviart_CMAME_1973_v2_p17}. In this paper, the 
authors have shown that acute-angle triangulation is a sufficient 
condition for a low-order approximation to satisfy maximum 
principles and the non-negative constraint. However, this 
condition is not sufficient under a high-order approximation. 
Other notable works on discrete maximum principles for high-order 
approximation are \cite{Hohn_Mittelmann_Computing_1981_v27_p145,
Yanik_ComputMathAppl_1989_v17_p1431,Solin_Vejchodsky_Araiza_MCS_2007_v76_p205,
Solin_Vejchodsky_JCAM_2007_v209_p54,Vejchodsky_Solin_MathComput_2007_v76_p1833}. 
All these works considered one-dimensional problems. Herein we systematically 
study the performance of high-order approximations on several two-dimensional 
problems. 

Also, earlier numerical works on discrete maximum principles 
concentrated on single-field formulations 
\cite{Nagarajan_Nakshatrala_IJNMF_2010}, and mixed formulations 
based on the variational multiscale formalism or lowest-order 
Raviart-Thomas spaces \cite{Nakshatrala_Valocchi_JCP_2009_v228_p6726}. 
Herein, we shall also investigate the performance of mixed formulations 
based on the least-squares formalism. 

%==========================================;
%  Subsection: Least-squares formulations  ;
%==========================================;
\subsection{Least-squares formulations}
Least-squares variational methods often constitute an appealing alternative 
to the more popular weak formulation based on the Galerkin formalism in 
developing efficient and robust finite element models. In a least-squares-based 
formulation a non-physical \textit{least-squares} functional is defined in terms 
of the sum of the squares of appropriate norms of the governing partial 
differential equation residuals. Since the least-squares functional is by 
definition positive and convex and it naturally follows that the minimizer 
of the least-squares functional coincides with the exact solution of the 
original set of partial differential equations.  The finite element model 
associated with the least-squares formulation is constructed via direct 
minimization of the least-squares functional with respect to the trial space 
associated with the finite element discretization. Some representative 
references on least-squares formulations are \cite{Bochev_Gunzburger,
Jiang_LSFEM}. 

%================================================;
%  Subsection: Main contributions of this paper  ;
%================================================;
\subsection{Main contributions of this paper} 
The main aim of this paper is to document the performance of 
$p$-refinement for solving diffusion-type equations with respect 
to maximum principles and the non-negative constraint. We 
illustrate the performance on various computational grids 
and using different canonical problems. We consider three 
weak formulations: the standard single-field formulation and 
two least-squares-based formulations. We illustrate the extent 
to which these formulations violate maximum principles and the 
non-negative constraint under high-order approximations. We do 
not, however, provide a methodology for enforcing maximum 
principles and the non-negative constraint under high-order 
approximations. We also show that the performance of 
least-squares formulations with respect to the non-negative 
constraint depends on the choice of the weight in the inner 
product.
%
The present work has two main purposes. First, users of 
high-approximations will be aware of their performance with 
respect to maximum principles and the non-negative constraint. 
Second, it will help researchers to develop methodologies for 
enforcing maximum principles and the non-negative under 
high-order approximations. 

%=======================================;
%  Subsection: An outline of the paper  ;
%=======================================;  
\subsection{An outline of the paper} 
The remainder of this paper is organized as follows. In Section 
\ref{Sec:S2_LS_DMP_Governing_equations}, we present the governing 
equations of anisotropic diffusion with decay. We shall also discuss 
the classical maximum principle, and its consequences (in particular, 
the non-negative constraint). In Section \ref{Sec:S3_LS_DMP_Weak_formulations}, 
we present the weak formulations, and in Section \ref{Sec:S4_LS_DMP_High_order} 
we discuss high-order spectral approximations. In Section 
\ref{Sec:S5_LS_DMP_Numerical_Results}, we shall show the performance 
of these numerical formulations using several canonical problems, and 
conclusions are drawn in Section \ref{Sec:S6_LS_DMP_Conclusions}. 

We shall employ the following symbolic notation in this paper. To 
distinguish vectors in the continuum setting from vectors in the finite 
element context, we shall employ lower case boldface normal letters 
for the former, and lower case boldface italic letters for the later. For 
example, $\mathbf{x}$ is used to denote a spatial position vector, and 
$\boldsymbol{c}$ is used to denote a finite element vector containing 
nodal concentrations. To distinguish a second-order tensor from a matrix, 
we shall denote second-order continuum tensors using upper case boldface 
normal letters, and shall denote matrices using upper case boldface italic 
letters. For example, $\mathbf{D}$ is used to denote the diffusivity 
tensor, and $\boldsymbol{K}$ is used to denote stiffness matrix. 
Throughout this paper, repeated indices do not imply summation. 
(That is, Einstein's summation convention is \emph{not} employed.)  
We shall denote the set of natural numbers as $\mathbb{N}$, and 
the set of real numbers as $\mathbb{R}$. Other notational conventions 
are introduced as needed. 

==> Sections/S2_LS_DMP_Governing_Equations.tex <==
%************************************************;
%                                                ;
%  Name                                          ;
%    S2_LS_DMP_Governing_Equations.tex           ;
%                                                ;
%************************************************;
\section{GOVERNING EQUATIONS: DIFFUSION WITH DECAY}
\label{Sec:S2_LS_DMP_Governing_equations}
In this paper, we assume that $\Omega$ is an open bounded subset
of $\mathbb{R}^{nd}$, where ``$nd$" denotes the number of spatial
dimensions.  The boundary is denoted by $\partial \Omega := \bar{\Omega}
- \Omega$, where a superposed bar denotes the set closure. The boundary 
is divided into two parts: $\Gamma^{\mathrm{D}}$ and $\Gamma^{\mathrm{N}}$, 
where $\Gamma^{\mathrm{D}}$ is that part of the boundary on which Dirichlet
boundary conditions are prescribed, and $\Gamma^{\mathrm{N}}$ is
the part of the boundary on which Neumann boundary conditions are 
prescribed. For well-posedness, we have $\Gamma^{\mathrm{D}} \cup
\Gamma^{\mathrm{N}} = \partial \Omega$ and $\Gamma^{\mathrm{D}}\cap
\Gamma^{\mathrm{N}} = \varnothing $. A spatial point is denoted by
$\mathbf{x} \in \bar{\Omega}$.  The gradient and divergence operators 
with respect to $\mathbf{x}$ are, respectively, denoted by $\mathrm{grad}
[\cdot]$ and $\mathrm{div}[\cdot]$. Herein, we shall consider the
anisotropic diffusion of a chemical species, and allow the decay 
of the chemical species. Let us denote the concentration of the 
chemical species by $c(\mathbf{x})$. 
%
We present the governing equations in the standard divergence 
form, which take the following form:
%----------------------------------------------;
%  Equation: Anisotropic diffusion with decay  ;
%----------------------------------------------;
\begin{subequations}
  \label{Eqn:LS_DMP_Governing_equations}
  \begin{alignat}{2}
    \label{Eqn:LS_DMP_diffusion_with_decay}
    &\alpha(\mathbf{x}) c(\mathbf{x}) - \mathrm{div}[\mathbf{D}(\mathbf{x})
      \mathrm{grad}[c]] = f(\mathbf{x}) & \qquad & \mathrm{in}
      \; \Omega  \\
    %
    &c(\mathbf{x}) = c^{\mathrm{p}} (\mathbf{x}) & \qquad &
    \mathrm{on} \; \Gamma^{\mathrm{D}} \\
    %
     \label{Eqn:LS_DMP_Neumann_BC}
    &\mathbf{n}(\mathbf{x}) \cdot \mathbf{D}(\mathbf{x}) \mathrm{grad}[c] =
    t^{\mathrm{p}}(\mathbf{x}) & \quad & \mathrm{on} \;
    \Gamma^{\mathrm{N}}
  \end{alignat}
\end{subequations}
%
where $\alpha(\mathbf{x}) \geq 0$ is the decay coefficient, $\mathbf{D}
(\mathbf{x})$ denotes the diffusivity tensor, $f(\mathbf{x})$ is the
volumetric source/sink, $c^{\mathrm{p}}(\mathbf{x}) $ is the prescribed
concentration, $t^{\mathrm{p}}(\mathbf{x})$ is the prescribed flux,
and $\mathbf{n}(\mathbf{x})$ is the unit outward normal vector on
the boundary. The mathematical model given by equations 
\eqref{Eqn:LS_DMP_diffusion_with_decay}--\eqref{Eqn:LS_DMP_Neumann_BC} 
frequently arises in Mathematical Physics (see the discussion in 
\cite[Introduction]{Nagarajan_Nakshatrala_IJNMF_2010}).

We shall assume that the decay coefficient is bounded above, which 
means that there exists a real constant $\alpha_0 < +\infty$ such 
that we have
%------------------------------------------------;
%  Equation: Decay coefficient is bounded above  ;
%------------------------------------------------;
\begin{align}
  \alpha(\mathbf{x}) < \alpha_0 \quad \forall \mathbf{x} \in \Omega
\end{align}
%
(Note that we have already assumed that the decay coefficient is
non-negative.) The diffusivity tensor is assumed to be symmetric,
bounded above and uniformly elliptic. That is, there exists two
constants $0 < \lambda_1 \leq \lambda_2 < +\infty$ such that
%---------------------------------------------------;
%  Equation: Diffusivity tensor uniformly elliptic  ;
%---------------------------------------------------;
\begin{align}
  \lambda_1 \mathbf{y}^{T} \mathbf{y} \leq \mathbf{y}^{T}
  \mathbf{D}(\mathbf{x}) \mathbf{y} \leq \lambda_2 \mathbf{y}^{T}
  \mathbf{y} \quad \forall \mathbf{x} \in \Omega , \; \forall
  \mathbf{y} \in \mathbb{R}^{nd}
\end{align}
%
It should be noted that uniform ellipticity condition is a stronger 
requirement than demanding that the matrix corresponding to tensor 
$\mathbf{D}(\mathbf{x})$ being positive definite at every spatial 
point in the domain. The system of equations 
\eqref{Eqn:LS_DMP_diffusion_with_decay}--\eqref{Eqn:LS_DMP_Neumann_BC} 
is a second-order elliptic partial differential equation with Dirichlet 
and Neumann boundary conditions. It is well-known that the above partial 
differential equation satisfies the so-called \emph{maximum principles} 
under certain regularity assumptions on the domain and on the input data 
($\mathbf{D}(\mathbf{x})$, $\alpha(\mathbf{x})$, $f(\mathbf{x})$, 
$c^{\mathrm{p}}(\mathbf{x})$, and $t^{\mathrm{p}}(\mathbf{x})$).

%==================================================================;
%  Subsection: Maximum principles and the non-negative constraint  ;
%==================================================================;
\subsection{Maximum principles and the non-negative constraint}
There are different kinds of maximum principles for second-order elliptic
partial differential equations available in the literature (for example, see 
the discussion in Han and Lin \cite{Han_Lin}). Herein, we consider two 
maximum principles by E.~Hopf \cite{Hopf_1927_v19_p147}. (Also see 
the commentary on Hopf's paper by J.~Serrin \cite{Serrin_AMS_2002}.)
The first maximum principle is for pure diffusion without decay (that is, 
$\alpha(\mathbf{x}) = 0$), and the second maximum principle allows 
the possibility of decay (that is, $\alpha(\mathbf{x}) \geq 0$). For $k 
\in \mathbb{N}$, we shall use $C^{k}(\Omega)$ to denote the set of 
functions having all derivatives up to the order $k$ continuous on 
$\Omega$, and $C^{0}(\bar{\Omega})$ to denote the space of all 
continuous functions on $\Omega$ that can be continuously 
extended to the boundary.

%---------------------------;
%  Theorem: Pure diffusion  ;
%---------------------------;
\begin{theorem}[A maximum principle for diffusion equation]
\label{Theorem:LS_DMP_MP_diffusion}
  Let $c(\mathbf{x}) \in C^{2}(\Omega) \cap C^{0}(\bar{\Omega})$ 
  satisfy the following differential inequality
  \begin{align*}
    -\mathrm{div}[\mathbf{D}(\mathbf{x}) \mathrm{grad}[c]] 
    = f(\mathbf{x}) \leq 0
  \end{align*}
  % 
  with $\mathbf{D}(\mathbf{x})$ is uniformly elliptic, bounded
  above and continuously differentiable. Then, we have
  \[
  \mathop{\mathrm{max}}_{\mathbf{x} \in \Omega} \;
  c(\mathbf{x}) \leq \mathop{\mathrm{max}}_{\mathbf{x} \in \bar{\Omega}}
  \; c(\mathbf{x})
  \]
\end{theorem}
%---------------------------------;
%  Theorem: Diffusion with decay  ;
%---------------------------------;
\begin{theorem}[A maximum principle for diffusion with decay]
\label{Theorem:LS_DMP_MP_diffusion_decay}
  Let $c(\mathbf{x}) \in C^{2}(\Omega) \cap C^{0}(\bar{\Omega})$ satisfy
  the following differential inequality
  \begin{align*}
    \alpha(\mathbf{x}) c(\mathbf{x}) -\mathrm{div}[\mathbf{D}
    (\mathbf{x}) \mathrm{grad}[c]] = f(\mathbf{x}) \leq 0
  \end{align*}
  %
  with $\alpha(\mathbf{x}) \geq 0$; $\mathbf{D}(\mathbf{x})$
  is uniformly elliptic, bounded above and continuously
  differentiable; and $\alpha(\mathbf{x})$ is bounded.
  Then, we have
  \[
  \mathop{\mathrm{max}}_{\mathbf{x} \in \Omega} \;
  c(\mathbf{x}) \leq \mathop{\mathrm{max}}_{\mathbf{x}
  \in \bar{\Omega}} \; \{c(\mathbf{x}),0\}
  \]
\end{theorem}
%
Mathematical proofs to the above two theorems can be found in Gilbarg 
and Trudinger \cite{Gilbarg_Trudinger}. In both theorems, we have 
assumed volumetric sink (i.e., $f(\mathbf{x}) \leq 0$). If we have 
volumetric source (i.e., $f(\mathbf{x}) \geq 0$) then the ``max" has 
to be replaced by ``min." Put differently, for volumetric source, the 
minimum occurs on the boundary in the case of pure diffusion, and the 
non-negative occurs on the boundary in the case of diffusion with decay. 
Similarly, if $f(\mathbf{x}) = 0$, then both the maximum and minimum 
occur on the boundary in the case of pure diffusion, and the non-negative 
maximum and non-negative minimum occur on the boundary in the case of 
diffusion with decay. If there are regions of both source and sink in 
the domain then the above theorems do not directly apply. The discrete 
version of maximum principles is commonly referred to as discrete 
maximum principles. 

There are several studies on discrete maximum principles, and some 
representative ones are \cite{Christie_Hall_IJNME_1984_v20_p549,
Kuzmin_Turek_JCP_2002_v175_p525,
Herrera_Valocchi_GW_2006_v44_p803,
Lipnikov_Shashkov_Svyatskiy_Vassilevski_JCP_2007_v227_p492,
Liska_Shashkov_CiCP_2008_v3_p852,
Nakshatrala_Valocchi_JCP_2009_v228_p6726,
Nagarajan_Nakshatrala_IJNMF_2010}.
%
Some of these studies (particularly the ones that derive necessary and 
sufficient conditions to meet the non-negative constraint and maximum 
principles, for example, references \cite{Kuzmin_Turek_JCP_2002_v175_p525}) 
hinge on the following mathematical arguments. After spatial discretization 
using the finite element method (or, for that matter, using the finite volume 
method or finite difference method) one obtains a system of linear equations 
of the following form:
%----------------------------------------;
%  Equation: System of linear equations  ;
%----------------------------------------;
\begin{align}
  \boldsymbol{A} \boldsymbol{x} = \boldsymbol{b}
\end{align}
%
where $\boldsymbol{A}$ is called the coefficient matrix, and 
$\boldsymbol{b}$ is called the force matrix. 
%
Under the low-order approximation (i.e., $ p = 1$), it can be shown 
that $\boldsymbol{b} \succeq \boldsymbol{0}$ if the forcing function 
$f(\mathbf{x}) \geq 0$. (Herein, we have used the symbol $\succeq$ 
to denote component-wise inequality. That is, $\boldsymbol{b} \succeq 
\boldsymbol{0}$ means that $b_i \geq 0$.) If $\boldsymbol{b} \succeq 
\boldsymbol{0}$, a sufficient condition for $\boldsymbol{x} \succeq 
\boldsymbol{0}$ is requiring the matrix $\boldsymbol{A}$ to be monotone 
(which means that the inverse of $\boldsymbol{A}$ has all non-negative 
entries). Usually, a stronger condition requiring that the matrix $\boldsymbol{A}$ 
is an M-matrix is commonly employed \cite{Kuzmin_Turek_JCP_2002_v175_p525}. 
(There are different ways of defining an M-matrix, and for further details 
see references \cite{Bapat_Raghavan,Saad}.) Restrictions are then placed 
(typically on the mesh) to make $\boldsymbol{A}$ to be an M-matrix. However, 
as discussed in references \cite{Nakshatrala_Valocchi_JCP_2009_v228_p6726} 
and \cite{Nagarajan_Nakshatrala_IJNMF_2010}, such a procedure will work 
only for isotropic diffusion, and is not sufficient for anisotropic 
diffusion. Several examples are presented in these two references 
to illustrate this conclusion.

For high-order approximations, another complexity arises due to the 
fact that even if $f(\mathbf{x}) \geq 0 \; \forall \mathbf{x} \in 
\Omega$, its $L_2$ projection onto the polynomial space need not 
be non-negative. That is, even if $f(\mathbf{x}) \geq 0$, the 
condition $\boldsymbol{b} \succeq \boldsymbol{0}$ need not hold 
under high-order approximations. Hence, the whole analysis requiring 
that $\boldsymbol{A}$ to be a monotone or an M-matrix will not 
guarantee that the non-negative constraint and maximum principles 
under high-order approximations will be met. In this paper, we 
carefully assess the performance of high-order approximations 
with respect to maximum principles and the non-negative 
constraint.   

%-------------------------------------------------;
%  Remark: Maximum principles for weak solutions  ;
%-------------------------------------------------;
\begin{remark}
  Some test problems in Section \ref{Sec:S5_LS_DMP_Numerical_Results} 
  do not have classical solutions in the sense that $c(\mathbf{x}) \in 
  C^{2}(\Omega) \cap C^{0}(\bar{\Omega})$, and hence, theorems 
  \ref{Theorem:LS_DMP_MP_diffusion} and \ref{Theorem:LS_DMP_MP_diffusion_decay} 
  do not directly apply. In the literature, however, one can find 
  maximum principles for weak solutions posed under weaker regularity 
  assumptions. For example, see references \cite{Pucci_Serrin,Chen_Wu,
    Borsuk_Kondratiev}. Such a detailed discussion is beyond the scope 
  of this paper, and is not central to our presentation.
\end{remark}

%------------------------------------;
%  Remark: Remark about prior works  ;
%------------------------------------;
\begin{remark}
  Some prior numerical works have addressed the non-negative 
  constraint and maximum principles for models similar to 
  equation \eqref{Eqn:LS_DMP_Governing_equations} on general 
  computational grids. Nakshatrala and Valocchi 
  \cite{Nakshatrala_Valocchi_JCP_2009_v228_p6726} have considered 
  discrete maximum principles for pure diffusion and two mixed 
  formulations. Specifically, they considered the variational 
  multiscale formulation and the lowest-order Raviart-Thomas 
  element. They provided a methodology for enforcing maximum 
  principles and the non-negative constraint that works only 
  for low-order finite elements. 
  %
  Nagarajan and Nakshatrala \cite{Nagarajan_Nakshatrala_IJNMF_2010} 
  have considered discrete maximum principles for the diffusion equation 
  with decay under the standard single-field formulation. They also 
  restricted their studies to low-order finite element approximations.  
  Liska and Shashkov \cite{Liska_Shashkov_CiCP_2008_v3_p852} have 
  addressed discrete maximum principles for pure diffusion using 
  conservative finite difference techniques. 
  %
   The present study differs from previous works in two ways: use 
   and performance study of (1) high-order approximations, and  
   (2)  least-squares finite element models.
  \end{remark} 

==> Sections/S3_LS_DMP_Weak_formulations.tex <==
%**********************************************;
%                                              ;
%  NAME                                        ;
%    S3_LS_DMP_Weak_formulations.tex           ;
%                                              ;
%**********************************************;
\section{WEAK FORMULATIONS}
\label{Sec:S3_LS_DMP_Weak_formulations}
In this paper we shall consider three weak formulations. The 
first is the classical single-field formulation, which is 
based on the Galerkin formalism. The second and third are 
mixed least-squares-based formulations. For completeness, 
we briefly outline these formulations. To this end, let 
us introduce the following function spaces:
%-----------------------------------------------------;
%  Equation: Function spaces in Galerkin formulation  ;
%-----------------------------------------------------;
\begin{subequations}
  \begin{align}
    \mathcal{U} &:= \left\{c(\mathbf{x}) \in H^{1}(\Omega) \; | \;
      c(\mathbf{x}) = c^{\mathrm{p}}(\mathbf{x}) \; \mathrm{on} \;
      \Gamma^{\mathrm{D}} \right\} \\
    %
    \mathcal{W} &:= \left\{w(\mathbf{x}) \in H^{1}(\Omega) \; | \;
      w(\mathbf{x}) = 0 \; \mathrm{on} \; \Gamma^{\mathrm{D}} \right\} \\
    %
    \mathcal{Q} &:= \left\{\mathbf{q}(\mathbf{x}) \; | \;
      \mathbf{q}(\mathbf{x}) \in (H^{1}(\Omega))^{nd}\right\}
  \end{align}
\end{subequations}
%
where $H^{1}(\Omega)$ is a standard Sobolev space \cite{Taylor_PDE_I}.
(Recall that ``$nd$'' denotes the number of spatial dimensions.)

%======================================================;
%  Subsection: The classical single-field formulation  ;
%======================================================;
\subsection{The classical single-field formulation}
The weak formulation based on the Galerkin formalism for the governing
equations
\eqref{Eqn:LS_DMP_diffusion_with_decay}-\eqref{Eqn:LS_DMP_Neumann_BC}
can be stated as follows: Find $c(\mathbf{x}) \in \mathcal{U} $ such
that we have
%---------------------------------------;
%  Equation: Galerkin weak formulation  ;
%---------------------------------------;
\begin{equation}
  \label{eq8}
  \mathcal{B}(w(\mathbf{x});c(\mathbf{x})) = \mathcal{F}
  (w(\mathbf{x})) \quad \forall w(\mathbf{x}) \in \mathcal{W}
\end{equation}
%
where the bilinear form $\mathcal{B}(w(\mathbf{x});c(\mathbf{x}))$
and the linear functional $\mathcal{F}(w(\mathbf{x}))$ are,
respectively, defined as follows:
%-------------------------------------------------;
%  Equation: Bilinear form and linear functional  ;
%-------------------------------------------------;
\begin{subequations}
  \label{eq9}
  \begin{align}
    \mathcal{B}(w(\mathbf{x});c(\mathbf{x})) &:= \int_{\Omega}
    \alpha(\mathbf{x}) w(\mathbf{x})c(\mathbf{x}) \; \mathrm{d}
    \Omega + \int_{\Omega} \mathrm{grad}[w]\cdot \mathbf{D}
    (\mathbf{x}) \mathrm{grad}[c] \; \mathrm{d} \Omega \\
    %
    \mathcal{F}(w(\mathbf{x})) &:= \int_{\Omega}  w(\mathbf{x})
    f(\mathbf{x}) \; \mathrm{d} \Omega  + \int_{\Gamma^{\mathrm{N}}}
    w(\mathbf{x}) t^{\mathrm{p}}(\mathbf{x}) \; \mathrm{d} \Gamma
  \end{align}
\end{subequations}
%
One can easily verify that the above weak formulation \eqref{eq8}
is equivalent to minimizing the following functional:
%-------------------------------------;
%  Equation: Minimization functional  ;
%-------------------------------------;
\begin{align}
  \label{eq10}
  \mathcal{J} (c(\mathbf{x}))
  &:= \frac{1}{2}\int_\Omega  {\Big( {\alpha(\mathbf{x}) c^2(\mathbf{x})
      + \mathrm{grad}[c] \cdot \mathbf{D}(\mathbf{x}) \mathrm{grad}[c]}
    \Big) \mathrm{d} \Omega} - \int_{\Omega}  c(\mathbf{x}) f(\mathbf{x})
  \; \mathrm{d} \Omega \notag \\
  &- \int_{\Gamma^{\mathrm{N}}} {c(\mathbf{x}) t^{\mathrm{p}}(\mathbf{x})
    \; \mathrm{d} \Gamma}
  = \frac{1}{2} \mathcal{B}(c(\mathbf{x});c(\mathbf{x}))
  - \mathcal{F}(c(\mathbf{x}))
\end{align}
%
Hence, the finite element approximation inherits the best approximation
property with respect to the norm $\left\| c \left( \mathbf{x} \right)
\right\|_E = \sqrt{\frac{1}{2} \mathcal{B}(c(\mathbf{x});c(\mathbf{x}))}$.

%================================================;
%  Subsection: Least-squares-based formulations  ;
%================================================;
\subsection{Least-squares-based formulations}
Least-squares variational procedures possess many attractive
mathematical as well as practical computational attributes.
In particular, the least-squares method always invokes a
minimization principle whose minimizer coincides with the
solution of the governing partial differential equations.
As a result, the discrete numerical solution always possesses
the best approximation property with respect to a well-defined
norm (i.e., the energy norm of the functional). When this norm
is equivalent to a standard norm (such as a norm from an appropriate
Sobolev space) ideal convergence rates of the finite element solution
may be established.  That the least-squares formulation is always based
on a minimization principle insures a robust setting that is often
lacking in the associated weak form Galerkin model.  In addition,
the bilinear form resulting from invocation of the minimization
principle in least-squares formulations will always be symmetric
and positive definite, and restrictive compatibility conditions
such as the \emph{inf-sup} condition will never arise.  As a result,
providing a conforming discretization and well-posed boundary
conditions, the discrete variational formulation will always possesses a unique solution.
Furthermore, the symmetry and positive-definiteness of the resulting coefficient matrix may
be exploited directly in the solution process of the linear system of equations.  In
particular, direct solvers may employ a sparse Cholesky decomposition of the coefficient
matrix, while iterative solvers may utilize the robust preconditioned conjugate gradient
algorithm.  Due to symmetry, only half of the coefficient matrix need to be actually calculated
and stored in memory.

Least-squares formulations are not without their own deficiencies and
in many cases there are fixes. For example, unlike weak form Galerkin
formulations where regularity requirements of the finite element spaces
are weakened (by invoking Green's identities), least-squares formulations
require higher regularity of the finite element spaces (dictated by the
order of the governing partial differential equations).  Higher regularity
requirements negatively affect the condition number of the coefficient
matrix and also the continuity requirement of the solution across element
boundaries. High regularity requirements may be avoided by constructing
the least-squares finite element model in terms of an equivalent lower-order
system by the introduction of additional independent variables. Such a mixed
formulation allows for the use of standard Lagrange interpolation functions 
but also produces a large set of global equations to be solved. Such a
formulation is often quite valuable, however, since the auxiliary variables
are typically physical quantities of interest such as the flux.

A least-squares-based formulation will be based on the minimization
of a least-squares functional, which is constructed from the sum of
the squares of appropriate norms of the residuals of the governing
partial differential equations and the Neumann boundary condition.
Although it is certainly possible to construct a least-squares
finite element model based on equations
\eqref{Eqn:LS_DMP_diffusion_with_decay}-\eqref{Eqn:LS_DMP_Neumann_BC}
directly, such an approach requires a higher degree of regularity in
the finite element solution such as $c(\mathbf{x}) \in H^2 \left(\Omega
\right)$, where $H^{2}(\Omega)$ is another standard Sobolev space
on $\Omega$ \cite{Taylor_PDE_I}. Herein, we recast the governing
equations into the following equivalent first-order system:
%------------------------------;
%  Equation: First-order form  ;
%------------------------------;
\begin{subequations}
  \label{eq13}
  \begin{alignat}{2}
    \label{Eqn:LS_DMP_mixed_decay}
    &\alpha(\mathbf{x}) c(\mathbf{x}) + \mathrm{div}[\mathbf{q}] =
    f(\mathbf{x}) & \quad & \mathrm{in} \; \Omega  \\
    %
    &\mathbf{q}(\mathbf{x}) = -\mathbf{D}(\mathbf{x}) \mathrm{grad}[c]
    & \quad & \mathrm{in} \; \Omega  \\
    %
    &c(\mathbf{x}) = c^{\mathrm{p}}(\mathbf{x}) & \quad & \mathrm{on} \;
    \Gamma^{\mathrm{D}} \\
    %
    \label{Eqn:LS_DMP_flux_BC}
    -&\mathbf{n}(\mathbf{x}) \cdot \mathbf{q}(\mathbf{x})
    = t^{\mathrm{p}}(\mathbf{x}) & \quad & \mathrm{on} \; \Gamma^{\mathrm{N}}
  \end{alignat}
\end{subequations}
%
where $\mathbf{q}(\mathbf{x})$ is the diffusive flux vector field. We shall
treat both $c(\mathbf{x})$ and $\mathbf{q}(\mathbf{x})$ as independent
variables, and employ the standard Lagrange finite element interpolation
functions for both of these field variables. The price incurred will be 
an increase in the overall size of the system of equations that one needs
to solve to obtain a numerical solution. The additional expense is not
unwarranted as the flux is an important quantity of interest in many
engineering applications. As a result, one obtains the flux directly
in the solution process as opposed to the usual way of obtaining it
at the post-processing stage of a finite element analysis.
%------------------------------------;
%  Remark: Remark of curl condition  ;
%------------------------------------;
\begin{remark}
For stability reasons, some least-squares formulations for diffusion-type 
equations augment the first order form of the governing partial differential 
equations (i.e., equations 
\eqref{Eqn:LS_DMP_mixed_decay}--\eqref{Eqn:LS_DMP_flux_BC}) 
with the following seemingly redundant expression:
%
\begin{align}
    \label{Eqn:LS_DMP_curl_q_condition}
    \mathrm{curl}[\mathbf{q}] = \mathbf{0}
  \end{align}
  %
 For example, see Reference \cite{Bochev_Gunzburger}. It is important to 
 note that $\mathbf{q}$ satisfies the above expression, in general, only if 
 the medium is homogeneous (that is, the diffusivity tensor is independent 
 of $\mathbf{x}$) and isotropic. In this work, we place no such restrictions 
 on $\mathbf{D}(\mathbf{x})$, and hence do not utilize the above expression 
 in construction of the least-squares functional.
 \end{remark}
%
We shall define the norm $\|\cdot\|_{K}$ for scalar and 
vector functions defined over $K$ as follows:
%-------------------------------------------------;
%  Equation: Norm on scalar and vector functions  ;
%-------------------------------------------------;
\begin{subequations}
  \begin{align}
    \|u(\mathbf{x})\|_{K}^{2} &:= \int_{K} u^{2}(\mathbf{x})
    \; \mathrm{d} K \\
    %
    \|\mathbf{u}(\mathbf{x})\|_{K}^{2} &:= \int_{K}
    \mathbf{u}(\mathbf{x}) \cdot \mathbf{u}(\mathbf{x})
    \; \mathrm{d} K
  \end{align}
\end{subequations}
%
In this paper we investigate the performance of two mixed
least-squares-based formulations, and denote them as ``LS1
formulation'' and ``LS2 formulation''. For both these
formulations, the least-squares functional can be
constructed as follows:
%--------------------------------------;
%  Equation: Least-squares functional  ;
%--------------------------------------;
\begin{align}
  \label{eq14}
  \mathcal{J}_{\mathrm{LS}} \left(c(\mathbf{x}),\mathbf{q}
    (\mathbf{x})\right)
  %
  &:= \frac{1}{2} \left\|\beta(\mathbf{x})\left(\alpha(\mathbf{x})
      c(\mathbf{x}) + \mathrm{div} \left[\mathbf{q} \right]
      - f(\mathbf{x}) \right) \right\|_{\Omega}^2 \nonumber \\
  %
  &+ \frac{1}{2} \left\|\mathbf{A}(\mathbf{x})
    \left(\mathbf{q}(\mathbf{x}) + \mathbf{D}(\mathbf{x})
      \mathrm{grad}[c] \right) \right\|_{\Omega}^2 \nonumber \\
  %
  &+ \frac{1}{2} \|\mathbf{q}(\mathbf{x}) \cdot \mathbf{n}
  (\mathbf{x}) + t^{\mathrm{p}}(\mathbf{x})\|^{2}_{\Gamma^{\mathrm{N}}}
\end{align}
%
where the second-order tensor $\mathbf{A}(\mathbf{x})$ and
the scalar function $\beta(\mathbf{x})$ are, respectively,
defined as follows:
%--------------------------------;
%  Equation: Definition of A(x)  ;
%--------------------------------;
\begin{subequations}
\label{Eqn:LS_DMP_lsfem_weights}
  \begin{align}
    \mathbf{A}(\mathbf{x}) &= \left\{
      \begin{array}{ll}
        \mathbf{I} & \mbox{LS1 formulation} \\
        \mathbf{D}^{-1/2}(\mathbf{x}) & \mbox{LS2 formulation} \\
      \end{array}\right. \\
    %
    \beta(\mathbf{x}) &= \left\{
      \begin{array}{cl}
        1 & \mbox{LS1 formulation} \\
        \left.
          \begin{array}{cl}
            1 & \mbox{if $\alpha(\mathbf{x}) = 0$} \\
            \alpha^{-1/2}(\mathbf{x}) & \mbox{if $\alpha(\mathbf{x}) \neq 0$}
          \end{array} \right\} & \mbox{LS2 formulation}
      \end{array} \right.
  \end{align}
\end{subequations}
%
where $\mathbf{I}$ is the second-order identity tensor. Recall 
that $\alpha(\mathbf{x}) \geq 0$, and hence $\beta(\mathbf{x})$ 
is well-defined. Also, note that $\mathbf{D}(\mathbf{x})$ is a 
positive definite tensor, and by square root theorem $\mathbf{D}^{-1/2}
(\mathbf{x})$ is also well-defined \cite{Gurtin}. The variational 
principle associated with both the least-squares formulations can 
be stated as follows: Find $c(\mathbf{x}) \in \mathcal{U}$ and 
$\mathbf{q}(\mathbf{x}) \in \mathcal{Q}$ such that we have
%--------------------------------------;
%  Equation: LS variational statement  ;
%--------------------------------------;
\begin{equation}
  \label{eq15}
  \mathcal{J}_{\mathrm{LS}}\left( c(\mathbf{x}),\mathbf{q}(\mathbf{x})
  \right) \leqslant \mathcal{J}_{\mathrm{LS}} \left(\tilde{c}(\mathbf{x}),
    \tilde{\mathbf{q}}(\mathbf{x})\right) \quad \forall \tilde{c}(\mathbf{x})
  \in \mathcal{U}, \; \tilde{\mathbf{q}}(\mathbf{x}) \in
  \mathcal{Q}
\end{equation}
%
The first-order optimality condition demands that the first
variation of $\mathcal{J}_{\mathrm{LS}} \left(c(\mathbf{x}),
  \mathbf{q}(\mathbf{x})\right) $ be identically zero. The
corresponding weak statement can be written as follows: Find
$c(\mathbf{x}) \in \mathcal{U}$ and $\mathbf{q}(\mathbf{x})
\in \mathcal{Q}$ such that we have
%----------------------------;
%  Equation: Weak statement  ;
%----------------------------;
\begin{equation}
  \label{Eqn:LS_DMP_weak_statement_LS}
  \mathcal{B}_{\mathrm{LS}} \left(w(\mathbf{x}),\mathbf{w}(\mathbf{x});
    c(\mathbf{x}),\mathbf{q}(\mathbf{x})\right)
  = \mathcal{F}_{\mathrm{LS}} \left(w(\mathbf{x}),
    \mathbf{w}(\mathbf{x})\right) \quad
  \forall w(\mathbf{x}) \in \mathcal{W}, \; \mathbf{w}(\mathbf{x})
  \in \mathcal{Q}
\end{equation}
%
where the bilinear form $\mathcal{B}_{\mathrm{LS}} \left(w(\mathbf{x}),
  \mathbf{w}(\mathbf{x}); c(\mathbf{x}), \mathbf{q}(\mathbf{x})\right)$
and the linear functional $\mathcal{F}_{\mathrm{LS}} \left(w(\mathbf{x}),
\mathbf{w}(\mathbf{x})\right)$ are, respectively, defined as follows:
%-------------------------------------------------;
%  Equation: Bilinear form and linear functional  ;
%-------------------------------------------------;
\begin{subequations}
  \label{eq17}
  \begin{align}
    \mathcal{B}_{\mathrm{LS}}\left(w(\mathbf{x}),\mathbf{w}(\mathbf{x});
      c(\mathbf{x}),\mathbf{q}(\mathbf{x})\right) &:=
    \int_{\Omega} \beta^{2}(\mathbf{x}) \left(\alpha(\mathbf{x}) w(\mathbf{x}) +
      \mathrm{div}[\mathbf{w}]\right) \left(\alpha(\mathbf{x})
      c(\mathbf{x}) + \mathrm{div}[\mathbf{q}] \right) \;
    \mathrm{d} \Omega \nonumber \\
    &+ \int_{\Omega} \left(\mathbf{w}(\mathbf{x}) + \mathbf{D}(\mathbf{x})
      \mathrm{grad}[w]\right) \cdot \mathbf{A}^{2}(\mathbf{x}) \left(\mathbf{q}
      (\mathbf{x}) + \mathbf{D}(\mathbf{x}) \mathrm{grad}[c] \right)
    \mathrm{d} \Omega \nonumber \\
    &+ \int_{\Gamma^{\mathrm{N}}} \mathbf{w}(\mathbf{x}) \cdot \mathbf{n}
    (\mathbf{x}) \; \mathbf{q} (\mathbf{x}) \cdot \mathbf{n}(\mathbf{x})
    \; \mathrm{d} \Gamma \\
    %
    \mathcal{F}_{\mathrm{LS}} \left(w(\mathbf{x}),\mathbf{w}(\mathbf{x})\right)
    &:= \int_{\Omega} \beta^{2}(\mathbf{x}) \left(\alpha(\mathbf{x})
      w(\mathbf{x}) + \mathrm{div}[\mathbf{w}] \right) f(\mathbf{x})
    \; \mathrm{d} \Omega - \int_{\Gamma^{\mathrm{N}}} \mathbf{w}(\mathbf{x})
    \cdot \mathbf{n} (\mathbf{x}) \; t^{\mathrm{p}}(\mathbf{x}) \;
    \mathrm{d} \Gamma
  \end{align}
\end{subequations}


==> Sections/S4_LS_DMP_High_order.tex <==
%************************************;
%                                    ;
%  NAME                              ;
%    S4_LS_DMP_High_order.tex        ;
%                                    ;
%************************************;
\section{HIGH-ORDER APPROXIMATIONS}
\label{Sec:S4_LS_DMP_High_order}
As shown in the previous section, a variational formulation (either Galerkin 
or least-squares formulations) of a general boundary value problem may 
be stated as follows: Find $\mathbf{u}(\mathbf{x}) \in \mathcal{V} $ such 
that we have
%
\begin{equation}
  \mathcal{B} \left({\mathbf{w (\mathbf{x})};\mathbf{u} (\mathbf{x})} 
  \right) = \mathcal{F} \left( \mathbf{w} (\mathbf{x}) \right) \quad 
  \forall \mathbf{w}(\mathbf{x}) \in \tilde{\mathcal{V}}
  \label{eq2}
\end{equation}
%
where $ \mathcal{B} \left( { \mathbf{w (\mathbf{x})};\mathbf{u} (\mathbf{x})} 
\right) $ is a bilinear form, $\mathcal{F} \left( \mathbf{w} (\mathbf{x}) 
\right) $ is a linear form, and $\mathcal{V}$ and $\tilde{\mathcal{V}}$ 
are appropriate function spaces. The quantity $ \mathbf{u} (\mathbf{x})$ 
represents the set of independent variables (associated with the variational 
boundary value problem), and $\mathbf{w}(\mathbf{x})$ represents the 
corresponding weighting function.

In the finite element method we restrict the solution space to a finite 
dimensional sub-space $\mathcal{V}^{hp}$ of the infinite dimensional 
space $ \mathcal{V}$, and the weighting functions to a finite dimensional 
sub-space $\tilde{\mathcal{V}}^{hp} \subset \tilde{\mathcal{V}}$. As a 
result, in the discrete case we seek to find $\mathbf{u}_{hp} (\mathbf{x}) 
\in \mathcal{V}^{hp} $ such that we have
%
\begin{equation}
  \mathcal{B} \left( { \mathbf{w}_{hp} (\mathbf{x}) ; \mathbf{u}_{hp} 
      (\mathbf{x})} \right) = \mathcal{F} \left( \mathbf{w}_{hp} 
    (\mathbf{x}) \right) \quad \forall \mathbf{w}_{hp}(\mathbf{x}) 
  \in \tilde{\mathcal{V}}^{hp}
  \label{eq3}
\end{equation}
%
We assume that the domain $ \bar \Omega \subset \mathbb{R}^{nd} $ is discretized 
into a set of NE non-overlapping sub-domains $ \bar \Omega^e $, called finite 
elements, such that $ \bar \Omega \approx \bar \Omega^ {hp} = \bigcup 
\nolimits_{e = 1}^{\text{NE}} {\bar \Omega }^e $.  The geometry of each 
${\bar \Omega^e} $ is characterized using the standard isoparametric bijective
mapping from $ {\bar \Omega^e} $ to the master element $ \hat \Omega^e $.  In the present study we 
restrict the classes of elements considered to lines in $ \mathbb{R} ^ 1 $, four side 
quadrilateral elements in $ \mathbb{R} ^ 2 $ and six face brick elements in 
$ \mathbb{R} ^ 3 $ (although numerical results are 
presented for $ nd = 1 $ and 2 only).  As a result we can simply define the master element as
$ {\hat \Omega^e} = [-1, +1]^{nd} $.  The natural coordinates associated with $ \hat \Omega^e $
(when $ nd = 3 $) are defined as $ \boldsymbol{\xi} = \left( {\xi ,\eta, \zeta } \right) $.
In this work we utilize a family of finite elements constructed using high polynomial order
interpolation functions.  The quantities $ h $ and $ p $ appearing in the definition of
the sub-space $ \mathcal{V}^{hp} $ imply that the discrete solution may be refined by either
increasing the number of elements in $ \bar \Omega ^ {hp} $ ($ h $-refinement), increasing the
polynomial order of the approximate solution within each element $ \bar \Omega ^ e $ ($ p $-refinement) or 
through an appropriate and systematic combination of both $ h $-refinement and $ p $-refinement.

Within a typical finite element a given variable, such as the species 
concentration $ c(\mathbf{x}) $, may be approximated by the following 
formula
%
\begin{equation}
  c\left( \mathbf{x} \right) \approx c_{hp} \left( \mathbf{x} \right) 
  = \sum\limits_{i = 1}^n {c_i^e{\psi _i}\left( \boldsymbol{\xi} \right)} 
  \quad \quad {\text{in }}{\hat \Omega ^e}
  \label{eq4}
\end{equation}

\noindent where $ {\psi _i} \left( \boldsymbol{\xi} \right) $ are the $ nd $-dimensional Lagrange
interpolation functions, $ c_i^e $ are the values of $ c_{hp}(\mathbf{x}) $ at the element nodes
and $ n = \left( p + 1 \right)^{nd} $ is the number of nodes in $ \hat \Omega^e $.  In addition, the
quantity $ p $ is the polynomial order of each interpolation function.  There are a variety
of ways in which high-order $ nd $-dimensional interpolation functions may be formulated.  For
our analysis we construct these polynomial functions from tensor products of the one-dimensional
$ C^0 $ spectral nodal interpolation functions

\begin{equation}
{\varphi _j}\left( \xi  \right) = \frac{{\left( {\xi  - 1} \right)\left( {\xi  + 1} \right){{L'}_p}\left( \xi  \right)}}
{{p\left( {p + 1} \right){L_p}\left( {{\xi _j}} \right)\left( {\xi  - {\xi _j}} \right)}}\quad \quad {\text{in }}\left[ { - 1, 1} \right]
\label{eq5}
\end{equation}

\noindent where $ L_p \left( \xi  \right) $ is the Legendre polynomial of order $ p $.  The
quantities $ {\xi _j} $ represent the locations of the nodes associated with the
one-dimensional interpolants (with respect to the natural coordinate $ \xi $).  The
one-dimensional nodal points are defined as the roots of the following expression

\begin{equation}
\left( {\xi  - 1} \right)\left( {\xi  + 1} \right){L'_p}\left( \xi  \right) = 0\quad \quad {\text{in }}\left[ { - 1, 1} \right]
\label{eq6}
\end{equation}
%
Figure \ref{Fig:LS_DMP_high_order_1D} compares high-order interpolation 
functions for $p = 6$ using uniform nodes with corresponding interpolation 
functions using non-uniform nodes based on Gauss-Lobatto-Legendre points. 

Multi-dimensional interpolation functions may be constructed from simple tensor products of the
one-dimensional spectral interpolants.  For example, in two-dimensions, the high-order
interpolation functions may be defined as

\begin{equation}
{\psi _i}\left( {\xi ,\eta } \right) = {\varphi _j}\left( \xi \right){\varphi _k}\left( \eta \right)
\quad \quad \text{in } \hat \Omega ^ e = \left[- 1, 1 \right] ^ 2
\label{eq7}
\end{equation}

\noindent where $ i = j + \left( k - 1 \right) \left( p + 1 \right) $ and $ j, k = 1,
\cdots, p + 1 $.  Likewise, in three-dimensions, the interpolants are expressed as

\begin{equation}
{\psi _i}\left( {\xi ,\eta ,\zeta } \right) = {\varphi _j}\left( \xi  \right){\varphi _k}\left( \eta  \right){\varphi _l}\left( \zeta  \right) \quad \quad {\text{in }} \hat \Omega ^ e = \left[- 1, 1 \right] ^ 3
\label{eq8}
\end{equation}

\noindent where $ i = j + \left[ k - 1 + \left( l - 1 \right) \left( p + 1 \right) \right]
\left( p + 1 \right) $ and $ j, k, l = 1, \cdots , p + 1 $.  Finite elements constructed
from tensor products of $ {\varphi _i}\left( \xi  \right) $ are commonly referred to as
spectral elements in the literature \cite{karniadakis:book}.  Such elements are merely
standard high order Lagrange type finite elements, where the locations of the unequally
spaced nodes in $ {\hat \Omega ^e} $ are taken as tensor products of the roots of 
equation \eqref{eq6}. 
%
Figure \ref{Fig:LS_DMP_high_order_2D} illustrates various examples of high-order 
two-dimensional elements. 

The finite element formulation naturally leads to a set of linear algebraic equations. The
resulting coefficient matrix and force vector associated with the equations are constructed
from the bilinear and linear forms appearing in equation \eqref{eq3} respectively. In this work
we utilize the standard Gauss-Legendre quadrature rules for numerical integration of these
quantities.  We utilize \textit{full integration} of all integrals and \textit{do not}
resort to selective under-integration of \textit{any} terms in the coefficient matrix or
force vector.  All numerical results have been obtained using a quadrature rule of at least 
$ \text{NGP} = p + 1 $, where NGP represents the number of quadrature points in the direction
of a given natural coordinate associated with $ \hat \Omega ^ e $.  For details on the
computer implementation of the finite element method, including descriptions of the bijective
isoparametric mapping $ {\bar \Omega ^e} \rightleftarrows {\hat \Omega ^e}$ and the global
assembly operator, we refer to the texts of Reddy \cite{reddy:fem} and Bathe \cite{bathe:book}.
For details on construction of the spectral interpolation functions, we refer to the book by
Karniadakis and Sherwin \cite{karniadakis:book}.


==> Sections/S5_LS_DMP_Numerical_Results_1D.tex <==
%***********************************************;
%                                               ;
%  NAME                                         ;
%    S5_LS_DMP_Numerical_Results.tex            ;
%                                               ;
%***********************************************;
\section{REPRESENTATIVE NUMERICAL RESULTS}
\label{Sec:S5_LS_DMP_Numerical_Results}
In this section, we illustrate the performance of high-order approximations
under the classical single-field formulation and two least-squares-based
formulations with respect to maximum principles and the non-negative
constraint. Before we present numerical results, we briefly discuss how
the numerical results under high-order approximations are visualized.

%========================================================================;
%  Subsection: Visualization of results using high-order approximations  ;
%========================================================================;
\subsection{Visualization of results using high-order approximations}
\label{Subsec:LS_DMP_visualization}
Once a numerical solution has been obtained using a particular finite 
element discretization, a given field variable may be evaluated at any 
point within a typical finite element using the standard interpolation 
formula given in equation \eqref{eq4}. Use of this formula is crucial 
in evaluating the performance of high-order finite element models with 
respect to maximum principles and the non-negative constraint. Unfortunately, 
it is typically impossible to employ this scheme explicitly in the actual 
visualization of multi-dimensional numerical results obtained using 
high-order spectral/\textit{hp} finite element formulations. 
%
Visualization software (such as Tecplot \cite{Tecplot360}) allow for the 
post-processing of structured data associated with a given finite element 
mesh; however, such programs typically require data structures containing 
the element connectivity array of low-order elements only. To utilize standard 
visualization software, it therefore becomes necessary to convert data 
associated with a high-order spectral/\textit{hp} finite element mesh into 
data associated with a low-order finite element mesh.

Solution data associated with a high-order finite element mesh may be readily 
converted into solution data associated with a low-order finite element 
discretization through the creation of a set of fictitious low-order 
visualization elements, utilized for plotting purposes only.  There are a 
variety of ways in which a low-order visualization mesh may be created.  
Perhaps, the simplest choice is to create a low-order mesh using only the 
actual nodes of the high-order finite element discretization.  Unfortunately, 
the visualized numerical results will inevitably deviate from the actual 
finite element solution within a given element when such an approach is 
taken.  In an effort to minimize visualization errors in the presentation of 
our numerical results, we utilize equation \eqref{eq4} to evaluate the numerical 
solution at a discrete number of points within a given element that is greater 
than the actual number of nodes of that element.  For one-dimensional 
problems, we simply interpolate the numerical solution onto 100 grid points 
within each finite element.  These grid points are then utilized explicitly to 
visualize the finite element solution.  For two-dimensional problems, equation 
\eqref{eq4} is again employed to evaluate the numerical solution at 256 
unequally spaced grid points within each element.  These points are the 
effective nodes associated with a spectral/\textit{hp} finite element using a 
15th order polynomial expansion (as geometrically characterized 
using the polynomial expansion associated with the actual element used in the 
numerical analysis). The refined set of points is then utilized to create a 
low-order visualization mesh that can be readily imported into Tecplot 
\cite{Tecplot360}. Alternatively, one can use any other procedure 
available in the literature for visualizing (scalar, vector and 
tensor) quantities interpolated using high-order approximations 
(for example, see \cite{Thompson_Pebay_SAND2005-6999,
Remacle_Chevaugeon_Marchandise_Geuzaine_IJNME_2007_v69_p750} 
and references therein). 

We now illustrate the performance of $p$- and $h$-refinements on 
various one- and two-dimensional test problems. For two-dimensional 
problems, the regions of the violation of the non-negative constraint 
are indicated using white color. 

%==================================================================;
%  Subsection: One-dimensional problem with zero forcing function  ;
%==================================================================;
\subsection{One-dimensional problem with zero forcing function}
\label{Subsec:LS_DMP_1D_zero_force}
This test problem is taken from Reference 
\cite{Nagarajan_Nakshatrala_IJNMF_2010}, which addressed the low-order 
approximation (i.e., $p = 1$). For completeness, we shall outline the problem. 
The domain is taken as $\Omega := (0,1)$ with zero forcing function and 
non-zero Dirichlet boundary conditions. Mathematically, the test problem 
can be written as follows:
%-------------------------------------;
%  Equation: One-dimensional problem  ;
%-------------------------------------;
\begin{subequations}
  \begin{align}
    \alpha c - \frac{d^2 c}{d \mathrm{x}^2} = 0
    \quad \mathrm{in} \; (0,1) \\
    %
    c(\mathrm{x} = 0) = c(\mathrm{x} = 1) = 1
  \end{align}
\end{subequations}
%
where $\alpha$ is a non-negative constant. The analytical
solution in terms of $\alpha$ is given by
%---------------------------------;
%  Equation: Analytical solution  ;
%---------------------------------;
\begin{align}
  c(\mathrm{x}) = \frac{1 - \exp[-\sqrt{\alpha}]}{\exp[\sqrt{\alpha}]
    - \exp[-\sqrt{\alpha}]} \exp[\sqrt{\alpha} \mathrm{x}] + \frac{\exp
    [\sqrt{\alpha}]-1}{\exp[\sqrt{\alpha}] - \exp[-\sqrt{\alpha}]}
  \exp[-\sqrt{\alpha} \mathrm{x}]
\end{align}
%
Herein we shall take $\alpha(\mathrm{x}) = 1000$. It should be noted
that the solution becomes steeper near the boundary as $\alpha$
becomes larger but the solution is still infinitely differentiable. The
computational mesh is obtained by discretizing the domain using
four equal-sized finite elements. The concentration profiles using
the single-field formulation and the two least-squares-based
formulations are, respectively, shown in Figures
\ref{Fig:LS_DMP_1D_Galerkin_conc}, \ref{Fig:LS_DMP_1D_first_LS_conc}
and \ref{Fig:LS_DMP_1D_second_LS_conc}. The flux profiles obtained
using the LS2 formulation (which is a least-squares-based mixed 
formulation) is shown in Figure \ref{Fig:LS_DMP_1D_no_forcing_flux}. 
%
In Reference \cite{Nagarajan_Nakshatrala_IJNMF_2010}, it has been 
shown that, for this test problem, the violation of the non-negative 
constraint vanishes with $h$-refinement under the classical single-field 
formulation. 
%
\emph{
From the numerical results presented in this subsection, one can 
conclude that the violation of the non-negative constraint also 
vanishes with $p$-refinement under the classical single-field and 
least-squares formulations for one-dimensional problems with zero 
forcing function.}

%======================================================================;
%  Subsection: One-dimensional problem with non-zero forcing function  ;
%======================================================================;
\subsection{One-dimensional problem with non-zero forcing function}
\label{Subsec:LS_DMP_1D_non_zero_force}
This test problem is taken from Reference
\cite{Solin_Vejchodsky_Araiza_MCS_2007_v76_p205}. Consider pure
diffusion (that is, decay is neglected) in domain $\Omega := (-1,1)$
with homogeneous Dirichlet boundary conditions. The forcing function
is taken to be
%------------------------------;
%  Equation: forcing function  ;
%------------------------------;
\begin{align}
  f(\mathrm{x}) = 200 \exp[-10(\mathrm{x} + 1)]
\end{align}
%
The test problem takes the following form:
%-------------------------------------;
%  Equation: One-dimensional problem  ;
%-------------------------------------;
\begin{subequations}
  \begin{align}
    -&\frac{d^2 c}{d \mathrm{x}^2} = f(\mathrm{x})
    \quad \mathrm{in} \; \Omega \\
    %
    &c(\mathrm{x} = -1) = c(\mathrm{x} = 1) = 0
  \end{align}
\end{subequations}
%
The analytical solution is given by
%---------------------------------;
%  Equation: Analytical solution  ;
%---------------------------------;
\begin{align}
  c(\mathrm{x}) = -2 \exp[-10(\mathrm{x} + 1)] -
  (1 - \exp[-20]) \mathrm{x} + (1 + \exp[-20])
\end{align}
%
We shall mesh the computational domain using one element, and solve 
the problem for various polynomial approximations in the element.
For this test problem, the LS1 and LS2 formulations are identical as 
$\alpha(\mathbf{x}) = 0$ and $\mathbf{D}(\mathbf{x}) = \mathbf{I}$. 
%
The obtained concentration profiles for various polynomial 
approximations under the classical single-field formulation 
and the least-squares formulations are shown in Figure 
\ref{Fig:LS_DMP_1D_homogeneous_Dirichlet}. Although for 
this problem $f(\mathbf{x}) \geq 0 \; \forall \mathbf{x} 
\in \Omega$, the classical single-field formulation (for 
$p = 3$) and the least-squares formulation (for $p = 3$ 
and $p = 5$) violate the non-negative constraint. The 
reason for the violation is that, under the classical 
single-field formulation, the $L_2$ projection of the 
forcing function onto the space spanned by $p = 3$ has 
negative values near $\mathrm{x} = 1$. A similar reason 
holds for the least-squares formulation.


==> Sections/S5_LS_DMP_Numerical_Results_2D.tex <==
%***********************************************;
%                                               ;
%  NAME                                         ;
%    S5_LS_DMP_Numerical_Results.tex            ;
%                                               ;
%***********************************************;
%===================================================;
%  Subsection: Two-dimensional isotropic diffusion  ;
%===================================================;
\subsection{Two-dimensional isotropic diffusion}
\label{Subsec:LS_DMP_2D_isotropic}
This test problem was proposed by Burman and Ern
\cite{Burman_Ern_CRM_2004_v338_p641}. The computational
domain is a rectangle $\Omega := (0,1) \times (0,0.3)$
with homogeneous Dirichlet boundary conditions. The decay
coefficient $\alpha(\mathbf{x})$ is taken to be zero. The
diffusivity tensor is the second-order identity tensor.
That is,
%--------------------------------;
%  Equation: Diffusivity tensor  ;
%--------------------------------;
\begin{align}
  \mathbf{D}(\mathbf{x}) = \mathbf{I}
\end{align}
%
The forcing function is taken as follows:
%------------------------------;
%  Equation: Forcing function  ;
%------------------------------;
\begin{align}
  f(\mathbf{x}) = \left\{\begin{array}{ll}
      1 & \mathrm{if} \; (\mathrm{x},\mathrm{y})
      \in [0,0.5] \times [0,0.075] \\
      0 & \mathrm{otherwise}
    \end{array} \right.
\end{align}
%
Since the forcing function $f(\mathbf{x}) \geq 0$ in $\Omega$ and
$c^{\mathrm{p}}(\mathbf{x}) = 0$ on $\partial \Omega$, from the maximum
principle given in Theorem \ref{Theorem:LS_DMP_MP_diffusion} we have
$c(\mathbf{x}) \geq 0$ in $\bar{\Omega}$. It should be noted that 
since the diffusivity tensor is isotropic and there is no decay, 
both the least-squares formulations are identical (see equation 
\eqref{Eqn:LS_DMP_lsfem_weights}). The computational and visualization 
meshes are shown in Figure \ref{Fig:LS_DMP_prob_3_mesh}. The concentration 
profiles obtained under the single-field and the least-squares formulations 
for various polynomial approximations are, respectively, shown in Figures 
\ref{Fig:LS_DMP_prob_3_weak_conc} and \ref{Fig:LS_DMP_prob_3_lsfem_conc}. 

The minimum concentration under the single-field and the least-squares 
formulations for various order of $p$- and $h$-refinements are given in 
Table \ref{Table:LS_DMP_problem_3_min_conc}. As one can see, there is 
violation of the non-negative constraint under $p$-refinement, and the 
violation vanishes under $h$-refinement. As discussed towards the end 
of Section \ref{Sec:S2_LS_DMP_Governing_equations}, the reason is that 
the $L_2$ projection of the forcing function on the polynomial space 
need not be non-negative under high-order approximations (even though 
the forcing function is non-negative). Note that the $L_2$ projection 
of the forcing function onto $p = 1$ polynomial space is non-negative. 

%---------------------------------------------;
%  Table: Concentration value for Problem #3  ;
%---------------------------------------------;
\begin{table}
  \centering
  \caption{Two-dimensional isotropic diffusion: This table 
    shows the variation of the minimum concentration with 
    respect to $p$-refinement and $h$-refinement. Since the 
    medium is isotropic, the violation of the non-negative 
    constraint vanishes with $h$-refinement. Although the 
    forcing function is non-negative, the violation of the 
    non-negative constraint did not vanish with $p$-refinement. 
    One of the reasons is that the $L_2$ projection of the 
    forcing function onto the polynomial space is \emph{not} 
    non-negative.\label{Table:LS_DMP_problem_3_min_conc}}
  \begin{tabular}{|c|c|c|c|c|} \hline
    \multirow{2}{*}{$h/p$ order} & \multicolumn{2}{|c|}{$p$-refinement} & \multicolumn{2}{|c|}{$h$-refinement} \\ 
    \cline{2-3} \cline{4-5}
    & Single-field & Least-squares & Single-field & Least-squares \\ \hline
    1  &  0                      &  0	                    &  0                      &    0                     \\
    2  &  $-1.35 \times 10^{-4}$  &  $-1.41 \times 10^{-4}$  &  $-8.84 \times 10^{-5}$  &  $-1.08 \times 10^{-4}$  \\
    3  &  $-3.13 \times 10^{-5}$  &  $-3.17 \times 10^{-5}$  &  $-1.81 \times 10^{-5}$  &  $-2.57 \times 10^{-5}$  \\
    4  &  $-2.04 \times 10^{-5}$  &  $-2.08 \times 10^{-5}$  &  0 & 0 \\
    5  &  $-4.42 \times 10^{-6}$  &  $-4.46 \times 10^{-6}$  &  0 & 0 \\ 
    6  &  $-2.77 \times 10^{-6}$  &  $-2.79 \times 10^{-6}$  &  0 & 0 \\
    7  &  $-1.99 \times 10^{-7}$  &  $-2.01 \times 10^{-7}$  &  0 & 0 \\
    8  &  $-6.22 \times 10^{-7}$  &  $-6.24 \times 10^{-7}$  &  0 & 0 \\
    9  &  $-2.60 \times 10^{-8}$  &  $-2.60 \times 10^{-8}$  &  0 & 0 \\
    10 &  $-2.06 \times 10^{-7}$  &  $-2.06 \times 10^{-7}$  &  0 & 0 \\ \hline
  \end{tabular}
\end{table}

%%======================================================================;
%%  Subsection: Diffusivity tensor from the subsurface flow literature  ;
%%======================================================================;
%\subsection{Diffusivity tensor from the subsurface flow literature}
%We shall assess the performance of $p$-refinement and the least-square
%formulation using a popular model for the diffusivity tensor, which is
%taken from the groundwater modeling literature (e.g., see Reference
%\cite{Pinder_Celia}). This particular diffusivity tensor has been
%also used in other numerical studies on discrete maximum principles
%and the non-negative constraint (for example, see References
%\cite{Herrera_Valocchi_GW_2006_v44_p803,
%Nakshatrala_Valocchi_JCP_2009_v228_p6726}).
%%
%The diffusivity tensor is given by
%%--------------------------------;
%%  Equation: Diffusivity tensor  ;
%%--------------------------------;
%\begin{align}
%  \mathbf{D}(\mathbf{x}) = \alpha_{T} \|\mathbf{v}\| \mathbf{I} +
%  \frac{\alpha_L - \alpha_T}{\|\mathbf{v}\|} \mathbf{v}
%  \otimes \mathbf{v}
%\end{align}
%%
%where $\mathbf{I}$ is the second-order identity tensor, $\otimes$
%is the tensor product, $\alpha_L$ and $\alpha_{T}$ are (respectively)
%the longitudinal and transverse diffusivity constants, and $\mathbf{v}
%(\mathbf{x})$ is a given velocity vector. (In groundwater modeling, the
%velocity vector is obtained by solving the governing equations for the
%flow, which is typically Darcy equation.) In various groundwater modeling
%applications, it is assumed that $\alpha_L \geq \alpha_{T}$.

%Herein, we shall use the aforementioned diffusivity tensor and
%solve a two-dimensional problem. The computational domain is a
%bi-unit square with homogeneous Dirichlet boundary conditions
%(i.e., $c^{\mathrm{p}}(\mathrm{x},\mathrm{y}) = 0$ on $\partial
%\Omega$), and the forcing function is given by
%%------------------------------;
%%  Equation: Forcing function  ;
%%------------------------------;
%\begin{align}
%  f(\mathrm{x},\mathrm{y}) = \left\{\begin{array}{ll}
%    1 & \mbox{if} \; (\mathrm{x},\mathrm{y}) \in [3/8,5/8]
%    \times [3/8,5/8] \\
%    0 & \mbox{otherwise}
%  \end{array} \right.
%\end{align}
%%
%The decay coefficient is taken to be zero. The following parameters are
%taken in the numerical simulation:
%%--------------------------------;
%%  Equation: Problem parameters  ;
%%--------------------------------;
%\begin{align}
%  \alpha_L = 0.1, \; \alpha_{T} = 0.01, \; \mathbf{v}
%  (\mathrm{x},\mathrm{y}) = \hat{\mathbf{e}}_{\mathrm{x}}
%  + \hat{\mathbf{e}}_{\mathrm{y}}
%\end{align}
%%
%where $\hat{\mathbf{e}}_{\mathrm{x}}$ and $\hat{\mathbf{e}}_{\mathrm{y}}$
%are the unit vectors along the $\mathrm{x}$- and $\mathrm{y}$-directions.

%=============================================;
%  Subsection: Non-uniform anisotropic media  ;
%=============================================;
\subsection{Non-uniform anisotropic media}
\label{Subsec:LS_DMP_non_uniform_anisotropic}
This test problem was originally proposed by Le Potier
\cite{LePotier_CRM_2005_v341_p787}, and has been employed 
in many other numerical studies on maximum principles and 
the non-negative constraint using the low-order approximation 
(e.g., see References \cite{Liska_Shashkov_CiCP_2008_v3_p852,
Nakshatrala_Valocchi_JCP_2009_v228_p6726}).
%
The test problem assumes $\alpha(\mathbf{x}) = 0$. The
computational domain is a square $\Omega := (0,0.5) \times
(0,0.5)$ with homogeneous Dirichlet boundary conditions
enforced on the whole boundary. The diffusivity tensor
is given by
\begin{align}
  \mathbf{D}(\mathbf{x}) = \left(
    \begin{array}{cc}
      \mathrm{y}^2 + \epsilon \mathrm{x}^2 & -(1 - \epsilon) \mathrm{x} \mathrm{y} \\
      -(1 - \epsilon) \mathrm{x} \mathrm{y} & \mathrm{x}^2 + \epsilon \mathrm{y}^2
    \end{array}\right)
\end{align}
%
with $\epsilon = 10^{-3}$. The forcing function is given by
\begin{align}
  f(\mathbf{x}) = \left\{
    \begin{array}{l}
      1 \quad (\mathrm{x},\mathrm{y}) \in [0.125,0.375] \times [0.125,0.375] \\
      0 \quad \mathrm{otherwise}
    \end{array}\right.
\end{align}
%
Two different meshes (one is a structured mesh and the 
other is an unstructured mesh) are employed, and are 
shown in Figures \ref{Fig:LS_DMP_prob_5_struct_mesh} 
and \ref{Fig:LS_DMP_prob_5_unstruct_mesh}. 
%
The performance of the single-field, LS1 and LS2 formulations using the 
structured mesh under both $p$- and $h$-refinements is illustrated in 
Figures \ref{Fig:LS_DMP_prob_5_struct_weak}, 
\ref{Fig:LS_DMP_prob_5_struct_lsfem_1} and 
\ref{Fig:LS_DMP_prob_5_struct_lsfem_2}. 
%
The performance of these formulations using the the unstructured 
mesh is illustrated in Figures \ref{Fig:LS_DMP_prob_5_unstruct_weak}, 
\ref{Fig:LS_DMP_prob_5_unstruct_LS1} and 
\ref{Fig:LS_DMP_prob_5_unstruct_LS2}. 
%
The minimum concentration under these three formulations is shown 
in Figure \ref{Fig:LS_DMP_prob_5_min_conc}. Since the anisotropy 
is strong, there will be violation of the non-negative constraint even 
on structured mesh for both $p$- and $h$-refinements. For this test 
problem, it should be noted that LS1 formulation did not perform as 
well as LS2 formulation. This is expected for problems involving 
heterogeneous and anisotropic media as the weight(s) in defining 
least-squares functional play a crucial role in the accuracy of the 
numerical results. (See equation \eqref{Eqn:LS_DMP_lsfem_weights} 
to note the different weights used in constructing LS1 and LS2 
formulations.)

%====================================================================;
%  Subsection: Anisotropic diffusion in a square domain with a hole  ;
%====================================================================;
\subsection{Anisotropic diffusion in a square domain with a hole}
\label{Subsec:LS_DMP_2D_hole}
This problem has been used in References
\cite{Liska_Shashkov_CiCP_2008_v3_p852,
Lipnikov_Shashkov_Svyatskiy_Vassilevski_JCP_2007_v227_p492,
Nakshatrala_Valocchi_JCP_2009_v228_p6726,
Nagarajan_Nakshatrala_IJNMF_2010}
with respect to the enforcement of the non-negative constraint 
but in the context of low-order approximation. The computational 
domain is a bi-unit square with a square hole of dimension $[4/9,5/9] 
\times [4/9,5/9]$. The forcing function is taken to be $f(\mathbf{x}) 
= 0$, and the decay coefficient is $\alpha(\mathbf{x}) = 0$. On the 
external boundary $c^{\mathrm{p}}(\mathbf{x}) = 0$ is prescribed, and 
on the internal boundary $c^{\mathrm{p}}(\mathbf{x}) = 2$ is prescribed. 
The diffusivity tensor is given by
\begin{align}
  \mathbf{D}(\mathbf{x}) =
  \left(\begin{array}{rr}
      \cos(\theta) & \sin(\theta) \\
      -\sin(\theta) & \cos(\theta)
    \end{array}\right)
  %
  \left(
    \begin{array}{cc}
      k_1 & 0 \\
      0 & k_2
    \end{array}
  \right)
  %
  \left(\begin{array}{rr}
      \cos(\theta) & -\sin(\theta) \\
      \sin(\theta) & \cos(\theta)
    \end{array}\right)
\end{align}
%
Herein, we have taken $\theta = \pi/6$, and considered two different 
sets for diffusivity coefficients: $(k_1,k_2) = (1,100)$ and $(k_1,k_2) 
= (1,10000)$.
%
The computational and visualization meshes are shown in Figure 
\ref{Fig:LS_DMP_prob_6_mesh}. The concentration profiles under 
the single-field, LS1 and LS2 formulations for various polynomial 
approximations are, respectively, shown in Figures 
\ref{Fig:LS_DMP_prob_6_k2_10000_Galerkin}, 
\ref{Fig:LS_DMP_prob_6_k2_10000_LS1}
and \ref{Fig:LS_DMP_prob_6_k2_10000_LS2}. 
%
Figure \ref{Fig:LS_DMP_prob_6_min_conc} shows the minimum concentration 
under these three formulations for both sets of diffusivity coefficients. 
From this figure, it is evident that the greater is disparity between the 
diffusivity coefficients $k_1$ and $k_2$ the greater is the violation of 
the non-negative constraint. Moreover, the extent of the violation did 
not decrease with with $p$- and $h$-refinements for strong anisotropic 
medium (see the case $k_1 = 1$ and $k_2 = 10000$). Hence, one can 
conclude that for strong anisotropic medium, $p$- and $h$-refinement 
do not eliminate the violation of the non-negative constraint.  

==> Sections/S6_LS_DMP_Conclusions.tex <==
%************************************************;
%                                                ;
%  NAME                                          ;
%    S6_LS_DMP_Conclusions.tex                   ;
%                                                ;
%  WRITTEN BY                                    ;
%    Kalyana Babu Nakshatrala                    ;
%                                                ;
%************************************************;
\section{CONCLUSIONS}
\label{Sec:S6_LS_DMP_Conclusions}
In this paper, we considered the diffusion-type equation, which is a 
second-order elliptic partial differential equation. This particular 
equation is known to satisfy maximum principles and the non-negative 
constraint under certain conditions. Many popular numerical formulations 
do not satisfy either maximum principles or the non-negative constraint. 
%
In the literature, it has been documented the performance of 
finite element formulations with respect to maximum principles 
for low-order elements. Herein, we considered the classical 
single-field formulation as well as two least-squares-based 
mixed formulations. We have systematically documented the 
performance of these formulations with respect to maximum 
principles and the non-negative constraint under high-order 
approximations.  
%
The main findings of this paper can be summarized as follows:
\begin{enumerate}[(a)]
  % 
\item For one-dimensional problems, it is well-known that a uniform 
  mesh is sufficient to satisfy the non-negative constraint and 
  maximum principles under the low-order approximation. (For 
  non-zero decay coefficient, the size of the element should 
  be smaller than a critical size.) However, a uniform mesh 
  is not sufficient for high-order approximations. (See 
  subsections \ref{Subsec:LS_DMP_1D_zero_force} and 
  \ref{Subsec:LS_DMP_1D_non_zero_force}.)
  % 
\item For isotropic two-dimensional problems, a well-centered triangular 
  mesh or a mesh with rectangular elements with aspect ratio between $1/
  \sqrt{2}$ and $\sqrt{2}$ is sufficient for the low-order approximation 
  to satisfy the non-negative constraint and maximum principles. Again, 
  these conditions are not sufficient for high-order approximations. 
  (See subsection \ref{Subsec:LS_DMP_2D_isotropic}.)
  % 
\item For anisotropic two-dimensional problems, any restrictions on the 
  mesh will not be sufficient, in general, to satisfy the non-negative 
  constraint and maximum principles for both low-order and high-order 
  approximations. (See subsections \ref{Subsec:LS_DMP_non_uniform_anisotropic} 
  and \ref{Subsec:LS_DMP_2D_hole}.)
  % 
\item The performance of a least-squares formulation depends on 
  the weight(s) used in defining the least-squares functional. 
  (See subsection \ref{Subsec:LS_DMP_non_uniform_anisotropic}, 
  and Figures \ref{Fig:LS_DMP_prob_5_struct_lsfem_1} and 
  \ref{Fig:LS_DMP_prob_5_unstruct_LS2}.)
  % 
\end{enumerate}	
%
We shall conclude this paper with the following statement with a hope 
that it will motivate applied mathematicians, computational mechanicians, 
and numerical analysts to work on an interesting problem: 
\emph{
A finite-element-based formulation or methodology that satisfies the 
non-negative constraint and maximum principles for anisotropic diffusion 
on general computational grids under high-order approximations is 
currently an unsolved problem with many important applications in 
engineering and applied sciences.}
